Actuarial Learning for Pension Fund Mortality Forecasting

For the assessment of the financial soundness of a pension fund, it is necessary to take into account mortality forecasting so that longevity risk is consistently incorporated into future cash flows. In this article, we employ machine learning models applied to actuarial science ({\it actuarial learning}) to make mortality predictions for a relevant sample of pension funds' participants. Actuarial learning represents an emerging field that involves the application of machine learning (ML) and artificial intelligence (AI) techniques in actuarial science. This encompasses the use of algorithms and computational models to analyze large sets of actuarial data, such as regression trees, random forest, boosting, XGBoost, CatBoost, and neural networks (eg. FNN, LSTM, and MHA). Our results indicate that some ML/AI algorithms present competitive out-of-sample performance when compared to the classical Lee-Carter model. This may indicate interesting alternatives for consistent liability evaluation and effective pension fund risk management.

==> Figuras/docs/f03db44f-31d6-47b1-894d-689fac8d5cab <==
{"id":"321241621323","lines":[{"id":"n0.3851416450923924","blocks":[],"style":{"align":"center"}},{"id":"n0.8036299509173257","blocks":[{"id":"n0.1587788430889272","text":"\\diagram","type":"composite","elements":{"de25841657518759065":{"id":"de25841657518759065","lines":[{"id":"n0.7382493169434772","blocks":[{"id":"n0.959444882036552","text":"2013"}]}],"shape":{"data":{"p":{"x":8,"y":41}},"anchor":"left-top"},"isTextMode":true},"de8914263482280762":{"id":"de8914263482280762","lines":[{"blocks":[{"text":"2014","id":"n0.4574068952999175"}],"id":"n0.6371329100868639"}],"shape":{"data":{"p":{"x":93,"y":39}},"anchor":"left-top"},"isTextMode":true},"de7811290142331586":{"id":"de7811290142331586","lines":[{"blocks":[{"text":"2015","id":"n0.5410018984621738"}],"id":"n0.5055359044382357"}],"shape":{"data":{"p":{"x":178,"y":38}},"anchor":"left-top"},"isTextMode":true},"de4205952310457015":{"id":"de4205952310457015","lines":[{"blocks":[{"text":"2016","id":"n0.9677659257619164"}],"id":"n0.1613266913223228"}],"shape":{"data":{"p":{"x":262,"y":38}},"anchor":"left-top"},"isTextMode":true},"de6169191389507886":{"id":"de6169191389507886","lines":[{"blocks":[{"text":"2017","id":"n0.7341658286123665"}],"id":"n0.49181599619973126"}],"shape":{"data":{"p":{"x":349,"y":36}},"anchor":"left-top"},"isTextMode":true},"de39603804412876875":{"id":"de39603804412876875","lines":[{"blocks":[{"text":"2018","id":"n0.3190116396857663"}],"id":"n0.12225391855649748"}],"shape":{"data":{"p":{"x":433,"y":36}},"anchor":"left-top"},"isTextMode":true},"de9699425384944858":{"id":"de9699425384944858","lines":[{"blocks":[{"text":"2019","id":"n0.9143800969892952"}],"id":"n0.6823800567560272"}],"shape":{"data":{"p":{"x":521,"y":35}},"anchor":"left-top"},"isTextMode":true},"de7631660458917109":{"id":"de7631660458917109","lines":[{"blocks":[{"text":"2013","id":"n0.09363336873185735"}],"id":"n0.08804107140587525"}],"shape":{"data":{"p":{"x":6,"y":109}},"anchor":"left-top"},"isTextMode":true},"de44491372436162036":{"id":"de44491372436162036","lines":[{"blocks":[{"text":"2014","id":"n0.31225255812443775"}],"id":"n0.9652144529362903"}],"shape":{"data":{"p":{"x":91,"y":107}},"anchor":"left-top"},"isTextMode":true},"de6774028687816216":{"id":"de6774028687816216","lines":[{"blocks":[{"text":"2015","id":"n0.19932240803806112"}],"id":"n0.7083825400448849"}],"shape":{"data":{"p":{"x":176,"y":106}},"anchor":"left-top"},"isTextMode":true},"de893059160590294":{"id":"de893059160590294","lines":[{"blocks":[{"text":"2016","id":"n0.9122707172438436"}],"id":"n0.799129672468448"}],"shape":{"data":{"p":{"x":260,"y":106}},"anchor":"left-top"},"isTextMode":true},"de5033550007178398":{"id":"de5033550007178398","lines":[{"blocks":[{"text":"2017","id":"n0.06863870683273743"}],"id":"n0.30742485248361295"}],"shape":{"data":{"p":{"x":347,"y":104}},"anchor":"left-top"},"isTextMode":true},"de18722728437986857":{"id":"de18722728437986857","lines":[{"blocks":[{"text":"2018","id":"n0.1313868158096354"}],"id":"n0.49167371672153926"}],"shape":{"data":{"p":{"x":431,"y":104}},"anchor":"left-top"},"isTextMode":true},"de35997354382301294":{"id":"de35997354382301294","lines":[{"blocks":[{"text":"2019","id":"n0.461469431579123"}],"id":"n0.20042529362331063"}],"shape":{"data":{"p":{"x":519,"y":103}},"anchor":"left-top"},"isTextMode":true},"de40735978967745967":{"id":"de40735978967745967","lines":[{"blocks":[{"text":"2013","id":"n0.7496434175259885"}],"id":"n0.046307013945001696"}],"shape":{"data":{"p":{"x":8,"y":185}},"anchor":"left-top"},"isTextMode":true},"de09088335965565308":{"id":"de09088335965565308","lines":[{"blocks":[{"text":"2014","id":"n0.6695665267080486"}],"id":"n0.04100521411864011"}],"shape":{"data":{"p":{"x":93,"y":183}},"anchor":"left-top"},"isTextMode":true},"de15177945505935386":{"id":"de15177945505935386","lines":[{"blocks":[{"text":"2015","id":"n0.3209590852455335"}],"id":"n0.6985676188495613"}],"shape":{"data":{"p":{"x":178,"y":182}},"anchor":"left-top"},"isTextMode":true},"de595829923214203":{"id":"de595829923214203","lines":[{"blocks":[{"text":"2016","id":"n0.3043303103621271"}],"id":"n0.4203483558490586"}],"shape":{"data":{"p":{"x":262,"y":182}},"anchor":"left-top"},"isTextMode":true},"de3972276281049385":{"id":"de3972276281049385","lines":[{"blocks":[{"text":"2017","id":"n0.20299137640592924"}],"id":"n0.5934377682995704"}],"shape":{"data":{"p":{"x":349,"y":180}},"anchor":"left-top"},"isTextMode":true},"de3176208345523521":{"id":"de3176208345523521","lines":[{"blocks":[{"text":"2018","id":"n0.9281970604837897"}],"id":"n0.2023001060517131"}],"shape":{"data":{"p":{"x":433,"y":180}},"anchor":"left-top"},"isTextMode":true},"de311906395083827":{"id":"de311906395083827","lines":[{"blocks":[{"text":"2019","id":"n0.3782822780791999"}],"id":"n0.6237907170698085"}],"shape":{"data":{"p":{"x":521,"y":179}},"anchor":"left-top"},"isTextMode":true},"de8551413592663415":{"id":"de8551413592663415","lines":[{"blocks":[{"text":"2013","id":"n0.09751995159072102"}],"id":"n0.42395904094225"}],"shape":{"data":{"p":{"x":10,"y":260}},"anchor":"left-top"},"isTextMode":true},"de8928266697249361":{"id":"de8928266697249361","lines":[{"blocks":[{"text":"2014","id":"n0.8680284816230308"}],"id":"n0.9647888263056559"}],"shape":{"data":{"p":{"x":95,"y":258}},"anchor":"left-top"},"isTextMode":true},"de3190798088142759":{"id":"de3190798088142759","lines":[{"blocks":[{"text":"2015","id":"n0.27723067170149807"}],"id":"n0.8546393414963842"}],"shape":{"data":{"p":{"x":180,"y":257}},"anchor":"left-top"},"isTextMode":true},"de8880852863197439":{"id":"de8880852863197439","lines":[{"blocks":[{"text":"2016","id":"n0.8509362069444866"}],"id":"n0.3367988267694051"}],"shape":{"data":{"p":{"x":264,"y":257}},"anchor":"left-top"},"isTextMode":true},"de9225290263352515":{"id":"de9225290263352515","lines":[{"blocks":[{"text":"2017","id":"n0.8513920708102589"}],"id":"n0.9435573212105706"}],"shape":{"data":{"p":{"x":351,"y":255}},"anchor":"left-top"},"isTextMode":true},"de23682382135878255":{"id":"de23682382135878255","lines":[{"blocks":[{"text":"2018","id":"n0.7046279442043286"}],"id":"n0.7803222547183146"}],"shape":{"data":{"p":{"x":435,"y":255}},"anchor":"left-top"},"isTextMode":true},"de40655466569523835":{"id":"de40655466569523835","lines":[{"blocks":[{"text":"2019","id":"n0.6910890058102293"}],"id":"n0.8115427163020164"}],"shape":{"data":{"p":{"x":523,"y":254}},"anchor":"left-top"},"isTextMode":true},"de743625051047133":{"id":"de743625051047133","lines":[{"id":"n0.6148456848429655","blocks":[{"id":"n0.21485951377367507","text":"Ano"}]}],"shape":{"data":{"p":{"x":603,"y":9}},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di868555879312038","items":[],"style":{}},"shapes":[{"id":"dp12513540730319228","type":"circle","data":{"p1":{"x":14.096588134765625,"y":11},"p2":{"x":40.375,"y":37.278411865234375}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp33446269701702414","type":"circle","data":{"p1":{"x":99.61079406738281,"y":10.278411865234375},"p2":{"x":125.88920593261719,"y":36.55682373046875}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp2508963399739541","type":"circle","data":{"p1":{"x":184.09658813476562,"y":10},"p2":{"x":210.375,"y":36.278411865234375}},"style":{"fillColor":[35,29,29,1]}},{"id":"da8005281033501026","data":[{"x":552.375,"y":20.139205932617188},{"x":600.1428527832031,"y":20.139205932617188}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dp37982539243496616","type":"circle","data":{"p1":{"x":354.6107940673828,"y":8.278411865234375},"p2":{"x":380.8892059326172,"y":34.55682373046875}},"style":{"fillColor":[235,235,235,1]}},{"id":"dp952742853865558","type":"circle","data":{"p1":{"x":439.0965881347656,"y":8},"p2":{"x":465.375,"y":34.278411865234375}},"style":{"fillColor":[235,235,235,1]}},{"id":"dp2410547121102422","type":"circle","data":{"p1":{"x":526.0965881347656,"y":7},"p2":{"x":552.375,"y":33.278411865234375}},"style":{"fillColor":[235,235,235,1]}},{"id":"dp6762717981254305","type":"flow-summing-junction","data":{"p1":{"x":268.75,"y":9.417617797851562},"p2":{"x":293.75,"y":35.41761779785156}},"style":{"fillColor":[0,0,0,0.49]}},{"id":"dp9503896834896572","type":"circle","data":{"p1":{"x":12.096588134765625,"y":79},"p2":{"x":38.375,"y":105.27841186523438}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp44558070482572143","type":"circle","data":{"p1":{"x":97.61079406738281,"y":78.27841186523438},"p2":{"x":123.88920593261719,"y":104.55682373046875}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp17209645236276083","type":"circle","data":{"p1":{"x":182.09658813476562,"y":78},"p2":{"x":208.375,"y":104.27841186523438}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp5590371198661466","type":"circle","data":{"p1":{"x":437.0965881347656,"y":76},"p2":{"x":463.375,"y":102.27841186523438}},"style":{"fillColor":[235,235,235,1]}},{"id":"dp36781137475130876","type":"circle","data":{"p1":{"x":524.0965881347656,"y":75},"p2":{"x":550.375,"y":101.27841186523438}},"style":{"fillColor":[235,235,235,1]}},{"id":"dp5539953202318046","type":"circle","data":{"p1":{"x":14.096588134765625,"y":155},"p2":{"x":40.375,"y":181.27841186523438}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp9952957981874522","type":"circle","data":{"p1":{"x":99.61079406738281,"y":154.27841186523438},"p2":{"x":125.88920593261719,"y":180.55682373046875}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp761302850143603","type":"circle","data":{"p1":{"x":184.09658813476562,"y":154},"p2":{"x":210.375,"y":180.27841186523438}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp2641627434013394","type":"circle","data":{"p1":{"x":526.0965881347656,"y":151},"p2":{"x":552.375,"y":177.27841186523438}},"style":{"fillColor":[235,235,235,1]}},{"id":"dp1700189705988866","type":"circle","data":{"p1":{"x":16.096588134765625,"y":230},"p2":{"x":42.375,"y":256.2784118652344}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp38010884954447044","type":"circle","data":{"p1":{"x":101.61079406738281,"y":229.27841186523438},"p2":{"x":127.88920593261719,"y":255.55682373046875}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp5265792366213613","type":"circle","data":{"p1":{"x":186.09658813476562,"y":229},"p2":{"x":212.375,"y":255.27841186523438}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp4023648465640466","type":"circle","data":{"p1":{"x":265.75,"y":77.27841186523438},"p2":{"x":292.0284118652344,"y":103.55682373046875}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp43998912214612473","type":"circle","data":{"p1":{"x":268.0965881347656,"y":153},"p2":{"x":294.375,"y":179.27841186523438}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp42101457717750024","type":"circle","data":{"p1":{"x":269.75,"y":228.27841186523438},"p2":{"x":296.0284118652344,"y":254.55682373046875}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp4683096464850527","type":"flow-summing-junction","data":{"p1":{"x":351.75,"y":77.41761779785156},"p2":{"x":376.75,"y":103.41761779785156}},"style":{"fillColor":[0,0,0,0.49]}},{"id":"dp4959617648488943","type":"circle","data":{"p1":{"x":353.75,"y":152.27841186523438},"p2":{"x":380.0284118652344,"y":178.55682373046875}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp45258882279678714","type":"circle","data":{"p1":{"x":355.75,"y":227.27841186523438},"p2":{"x":382.0284118652344,"y":253.55682373046875}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp04866148615009269","type":"circle","data":{"p1":{"x":441.75,"y":227.27841186523438},"p2":{"x":468.0284118652344,"y":253.55682373046875}},"style":{"fillColor":[35,29,29,1]}},{"id":"dp07849585585026997","type":"flow-summing-junction","data":{"p1":{"x":439.75,"y":152.41761779785156},"p2":{"x":464.75,"y":178.41761779785156}},"style":{"fillColor":[0,0,0,0.49]}},{"id":"dp8685919583225434","type":"flow-summing-junction","data":{"p1":{"x":527.75,"y":225.41761779785156},"p2":{"x":552.75,"y":251.41761779785156}},"style":{"fillColor":[0,0,0,0.49]}},{"id":"da9691871232261642","data":[{"x":41.18223571777344,"y":23.417617797851562},{"x":99.61079406738281,"y":23.417617797851562}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3831712087721728","data":[{"x":125.88920593261719,"y":23.417617797851562},{"x":184.31776428222656,"y":23.417617797851562}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3184887362222295","data":[{"x":210.375,"y":23.139205932617188},{"x":268.75,"y":23.139205932617188}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da4243352759421144","data":[{"x":293.75,"y":22.417617797851562},{"x":354.6107940673828,"y":22.417617797851562}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9855103597060733","data":[{"x":380.8892059326172,"y":21.417617797851562},{"x":439.2642059326172,"y":21.417617797851562}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da09410425210316231","data":[{"x":465.375,"y":21.139205932617188},{"x":526.0965881347656,"y":21.139205932617188}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da2260268846158291","data":[{"x":38.375,"y":92.13920593261719},{"x":96.80355834960938,"y":92.13920593261719}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5759524183598206","data":[{"x":40.375,"y":168.1392059326172},{"x":98.80355834960938,"y":168.1392059326172}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da060863444926603005","data":[{"x":42.375,"y":243.1392059326172},{"x":100.80355834960938,"y":243.1392059326172}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8755139612820957","data":[{"x":123.88920593261719,"y":91.41761779785156},{"x":182.31776428222656,"y":91.41761779785156}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9191300048219426","data":[{"x":125.88920593261719,"y":167.41761779785156},{"x":184.31776428222656,"y":167.41761779785156}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da16590931965923583","data":[{"x":127.88920593261719,"y":242.41761779785156},{"x":186.31776428222656,"y":242.41761779785156}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8457660768801081","data":[{"x":208.375,"y":91.13920593261719},{"x":266.8035583496094,"y":91.13920593261719}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9914701218344759","data":[{"x":210.375,"y":167.1392059326172},{"x":268.8035583496094,"y":167.1392059326172}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9973746074910941","data":[{"x":212.375,"y":242.1392059326172},{"x":270.8035583496094,"y":242.1392059326172}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da20521588401519253","data":[{"x":292.0284118652344,"y":90.41761779785156},{"x":351.75,"y":90.41761779785156}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da05108363320902898","data":[{"x":294.375,"y":166.1392059326172},{"x":353.75,"y":166.1392059326172}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8857608669659915","data":[{"x":296.0284118652344,"y":241.41761779785156},{"x":355.75,"y":241.41761779785156}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5112805271765748","data":[{"x":376.75,"y":89.13920593261719},{"x":437.0965881347656,"y":89.13920593261719}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9115735698062535","data":[{"x":380.0284118652344,"y":165.41761779785156},{"x":439.75,"y":165.41761779785156}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7851821194423716","data":[{"x":382.0284118652344,"y":240.41761779785156},{"x":441.75,"y":240.41761779785156}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da667896668217923","data":[{"x":463.375,"y":89.13920593261719},{"x":524.0965881347656,"y":89.13920593261719}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6698857686826765","data":[{"x":465.375,"y":165.1392059326172},{"x":526.0965881347656,"y":165.1392059326172}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9422960037498718","data":[{"x":468.0284118652344,"y":240.41761779785156},{"x":528.75,"y":240.41761779785156}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da903895203181907","data":[{"x":550.375,"y":88.13920593261719},{"x":598.1428527832031,"y":88.13920593261719}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da5366268380373564","data":[{"x":552.375,"y":164.1392059326172},{"x":600.1428527832031,"y":164.1392059326172}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da18125171513871452","data":[{"x":552.75,"y":238.41761779785156},{"x":600.5178527832031,"y":238.41761779785156}],"head":">","tail":"no","shaft":"-","mVer":1}],"settings":{"grid":false}}]},{"id":"n0.6923899984614412","blocks":[],"style":{"align":"center"}}],"pageSettings":{"pageSize":{"width":700}},"delayRenderCache":{"av":1380,"map":{}},"___version":2,"version":2,"av":1380}
